Measurement of the suppression and azimuthal anisotropy of muons from heavy-flavor decays in Pb+Pb collisions at $\sqrt{s_{\mathrm{NN}}} = 2.76$ TeV with the ATLAS detector

ATLAS measurements of the production of muons from heavy-flavor decays in $\sqrt{s_{\mathrm{NN}}} = 2.76$ TeV Pb+Pb collisions and $\sqrt{s} = 2.76$ TeV $pp$ collisions at the LHC are presented. Integrated luminosities of 0.14 $\mathrm{nb}^{-1}$ and 570 $\mathrm{nb}^{-1}$ are used for the Pb+Pb and $pp$ measurements, respectively, which are performed over the muon transverse momentum range $4 < p_{\mathrm{T}} < 14$ GeV and for five Pb+Pb centrality intervals. Backgrounds arising from in-flight pion and kaon decays, hadronic showers, and mis-reconstructed muons are statistically removed using a template-fitting procedure. The heavy-flavor muon differential cross-sections and per-event yields are measured in $pp$ and Pb+Pb collisions, respectively. The nuclear modification factor $R_{\mathrm{AA}}$ obtained from these is observed to be independent of $p_{\mathrm{T}}$, within uncertainties, and to be less than unity, which indicates suppressed production of heavy-flavor muons in Pb+Pb collisions. For the 10% most central Pb+Pb events, the measured $R_{\mathrm{AA}}$ is approximately 0.35. The azimuthal modulation of the heavy-flavor muon yields is also measured and the associated Fourier coefficients $v_n$ for $n =$ 2, 3 and 4 are given as a function of $p_{\mathrm{T}}$ and centrality. They vary slowly with $p_{\mathrm{T}}$ and show a systematic variation with centrality which is characteristic of other anisotropy measurements, such as that observed for inclusive hadrons. The measured $R_{\mathrm{AA}}$ and $v_n$ values are also compared with theoretical calculations.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 24-Oct-2018

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DRF/IRFU, France; SRNSFG, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, CANARIE, CRC and Compute Canada, Canada; COST, ERC, ERDF, Horizon 2020, and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d' Avenir Labex and Idex, ANR, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF, Greece; BSF-NSF and GIF, Israel; CERCA Programme Generalitat de Catalunya, Spain; The Royal Society and Leverhulme Trust, United Kingdom. 

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------


